Stabilization of Exoskeletons through Active Ankle Compensation

This paper presents an active stabilization method for a fully actuated lower-limb exoskeleton. The method was tested on the exoskeleton ATALANTE, which was designed and built by the French start-up company Wandercraft. The main objective of this paper is to present a practical method of realizing more robust walking on hardware through active ankle compensation. The nominal gait was generated through the hybrid zero dynamic framework. The ankles are individually controlled to establish three main directives; (1) keeping the non-stance foot parallel to the ground, (2) maintaining rigid contact between the stance foot and the ground, and (3) closing the loop on pelvis orientation to achieve better tracking. Each individual component of this method was demonstrated separately to show each component's contribution to stability. The results showed that the ankle controller was able to experimentally maintain static balance in the sagittal plane while the exoskeleton was balanced on one leg, even when disturbed. The entire ankle controller was then also demonstrated on crutch-less dynamic walking. During testing, an anatomically correct manikin was placed in the exoskeleton, in lieu of a paraplegic patient. The pitch of the pelvis of the exoskeleton-manikin system was shown to track the gait trajectory better when ankle compensation was used. Overall, active ankle compensation was demonstrated experimentally to improve balance in the sagittal plane of the exoskeleton manikin system and points to an improved practical approach for stable walking.

==> Sections/_CLF.tex <==
\section{Static Balance}
\label{sec:StaticBalance}
The proposed solution was first implemented to achieve static balance. This proves the stabilization method for a time-invariant system.

The system can be statically stabilized to a position other than the equilibrium point by shifting the equilibrium point of the system using the following formulation:
\begin{gather*}
    u = u_1 + u_{FF} \\
    \dot{x} = f(x) + g(x)u_1 + g(x)u_{FF} 
\end{gather*}
where $u_{FF}$ is the feed-forward control required to statically hold a position.

Control at the ankle was achieved using a control Lyapunov function quadratic program (CLF-QP) that optimizes for convergence rate of the CLF. A control lyapunov function was synthesized using the linearized system dynamics. It has been proven that a CLF synthesized using the continuous-time Lyapunov equation (CTLE) is a valid CLF. It remains to be proven that this CLF is locally valid for the nonlinear system. \\

\textbf{Proposition}: A CLF synthesized from linearized system dynamics is locally valid for the nonlinear system in a ball around the equilibrium point. 

Proof: Consider a candidate CLF synthesized from the CTLE, $V(x) = x^T P x$. This candidate CLF is a valid CLF for the linear system. Thus, it is given that:
\begin{gather*}
    c_1 ||x||^2 \leq V(x) \leq c_2||x||^2  \tag{ia}\\
    \inf_{u\in U}[L_AV(x) + L_BV(x)u] \leq -c_3 ||x|| \tag{iia}
\end{gather*} 
Thus, the CLF is valid for the nonlinear system if $\exists$ $c_1, c_2, c_3 > 0$ such that:
\begin{gather*}
    \inf_{u\in U}[L_fV(x) + L_gV(x)u] \leq -c_4 ||x|| \tag{iib}
\end{gather*}
Differentiating the candidate CLF for the nonlinear system dynamics yields:
\begin{align*}
    L_fV(x) + L_gV(x)u &= x^T P \dot{x} + \dot{x}^T P x
\end{align*}
The nonlinear system can be decomposed into a linear and a nonlinear component around the equilibrium point, $x_e$: 
\begin{gather*}
    \dot{x} = Ax + Bu + e(x,u) \\
    e(x,u) = f(x) + g(x)u - Ax - Bu
\end{gather*}
where $A, B$ provide a linear approximation of the nonlinear dynamics and $e(x,u)$ represents the error resulting from linearization. It is important to note that since the system was linearized around the equilibrium point, $e(x,u) = 0$ at the equilibrium point. Substituting the linearized dynamics into the:
\begin{align*}
    L_fV(x) + L_gV(x)u &= x^T P (Ax + Bu + e(x,u)) \\
                        &\quad + (Ax + Bu + e(x,u))^T P x \\
                        &= x^TP(Ax + Bu) + (Ax + Bu)^TPx \\
                        &\quad + 2x^TPe(x,u) \\
                        &= L_AV(x) + L_BV(x)u + 2x^TPe(x,u)
\end{align*}
Expanding condition (iib):
\begin{multline*}
    \inf_{u\in U}[L_fV(x) + L_gV(x)u] \\
    = \inf_{u\in U}[L_AV(x) + L_BV(x)u + 2x^TPe(x,u)] \\
    \leq -c_3||x|| + \inf_{u \in U}[2x^TPe(x,u)]
\end{multline*}
As stated before, the error term at the equilibrium point is zero. Thus, there exists an $r$ such that for all $x \in B_r(x_e)$, $||e(x)|| < c_5$. Thus, 
\begin{align*}
    \inf_{u\in U}[L_fV(x) + L_gV(x)u] &\leq -c_4||x|| 
\end{align*}
for the ball such that $c_5 = \frac{c_3}{2\lambda_{\max}(P)}$. Thus, there exists $r > 0$ such that $\forall x \in B_r(x_e)$, the CLF synthesized from the linearized dynamics is valid for the nonlinear system. \\ 

Since the CLF is locally valid for the nonlinear system, the system is controllable. Thus, a CLF-QP designed to actively control the ankle joints is fully controllable. The system can be modeled as a set of controllable and noncontrollable states.
\begin{align*}
    \dot{x} = f(x) + g(x)\begin{bmatrix} h(x) \\ u\end{bmatrix}
\end{align*}
where $u \in \mathbb{R}^2$ and $h(x) \in \mathbb{R}^{10}$ for the static CLF-QP. 
